Power handling in a highly-radiative negative triangularity pilot plant

This work explores power handling solutions for high-field, highly-radiative negative triangularity (NT) reactors based around the MANTA concept \cite{rutherford_manta_2024}. The divertor design is kept as simple as possible, opting for a standard divertor with standard leg length. FreeGS is used to create an equilibrium for the boundary region, prioritizing a short outer leg length of only $\sim$50 cm ($\sim$40\% of the minor radius). The UEDGE code package is used for the boundary plasma solution, to track plasma temperatures and fluxes to the divertor targets. It is found that for $P_\mathrm{SOL}$ = 25 MW and $n_\mathrm{sep} = 0.96 \times 10^{20}$ m$^{-3}$, conditions consistent with initial core transport modeling, little additional power mitigation is necessary. For external impurity injection of just 0.13\% Ne, the peak heat flux density at the more heavily loaded outer targets falls to 7.8 MW/m$^{2}$, while the electron temperature $T_\mathrm{e}$ remains just under 5 eV. Scans around the parameter space reveal that even at densities lower than in the primary operating scenario, $P_\mathrm{SOL}$ can be increased up to 50 MW, so long as a slightly higher fraction of extrinsic radiator is used. With less than 1\% neon (Ne) impurity content, the divertor still experiences less than 10 MW/m$^{2}$ at the outer target. Design of the plasma-facing components includes a close-fitting vacuum vessel with a tungsten inner surface as well as FLiBe-carrying cooling channels fashioned into the VV wall directly behind the divertor targets. For the seeded heat flux profile, Ansys Fluent heat transfer simulations estimate that the outer target temperature remains at just below 1550\degree C. Initial scoping of advanced divertor designs shows that for an X-divertor, detachment of the outer target becomes much simpler, and plasma fluxes to the targets drop considerably with only 0.01\% Ne content.

==> equ.tex <==
\label{sec:equ}

MANTA's magnetic equilibrium was first scoped with the Grad-Shafranov solver CHEASE\cite{LutjensCHEASE} before being further refined with another Grad-Shafranov solver, FreeGS\cite{FreeGS}, that is able to model the X-point and divertor region. As the final MANTA equilibrium was still evolving at the time of writing, an equilibrium generated by FreeGS for an earlier operating point is instead used. This equilibrium is shown in Fig. \ref{fig:freeGS_equi}, where parabolic fits were used for the current and pressure profiles generated by integrated modeling. Thus, while not the final MANTA design, it is still self-consistent and allows for representative scoping of divertor operation for negative triangularity tokamaks similar to MANTA.

The over-arching goal while designing the PF coilset in FreeGS was to keep the divertor as simple as possible, meaning no complex magnetic topologies and minimal X-points, while still surviving $P_{SOL} = 25$ MW. This resulted in four pairs of PF coils, which were placed inside the toroidal field (TF) coils to reduce their cost. This was possible because MANTA's TF coils are demountable, allowing access to their interior. The PF coil locations shown in Fig \ref{fig:freeGS_equi} were determined through moving the coils by hand and running neutronics simulations for each new coilset. Similarly to the equilibrium, these coils are not those of MANTA's final point design; the general trends and results presented below are not overly sensitive to the precise coil and equilibrium information.

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{images/endOfClassEqui.pdf}
\caption{The poloidal cross-section used in this work, which is modified slightly from the MANTA design presented in reference \cite{rutherford_manta_2024}.}
\label{fig:freeGS_equi}
\end{figure}

\begin{table}
\begin{center}
\caption{Poloidal field coil parameters}
\label{tab:PF_params}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllll}
 \hline
 Parameter & PF1 & PF2 & PF3 & PF4\\
 \hline
 \hline
Current $\cdot$turns [MA$\cdot$turns] & -7.8 & 6.1 & 2.1 & -4.3\\
Number of turns & 86 & 67 & 24 & 48\\
Height [m] & 0.33 & 0.29 & 0.14 & 0.29 \\
Width [m] & 0.37 & 0.33 & 0.22 & 0.22\\
R [m] & 3.65 & 5.05 & 6.25 & 6.65 \\
Z [m] & $\pm$2.25 & $\pm$2.9 & $\pm$2.5 & $\pm$ 1.25 \\
 \hline
\end{tabular}}
\end{center}
\end{table}
